The large-charge expansion in nonrelativistic conformal field theories

Conformal field theories (CFTs) are associated with critical phenomena and phase transitions and also play an essential role in string theory. Solving a CFT is an extremely constrained problem due to conformal invariance -- the task essentially reduces to the computation of a set of numbers called the CFT data -- yet it remains highly nontrivial. In fact, CFTs usually are strongly coupled and thus require new tools that do not rely on perturbation theory. For these reasons, in the past few decades, they became one of the most active fields of research. A natural extension of these ideas with far-reaching implications for condensed matter systems -- in which relativistic effects are not manifest -- is to replace the Poincare group by the Galilean group, thereby opening the way to a precise formulation of a whole new class of critical phenomena in terms of nonrelativistic conformal field theories (NRCFTs). Many of the aforementioned tools developed to gain a better formal understanding of CFTs can then be adapted to gain a strong predictive power in systems with direct experimental relevance. In recent years, a new powerful tool has emerged: the large-charge expansion. It allows to systemically uncover part of the CFT data of theories with global symmetries, thereby revealing profound and universal features of these systems. Using the state-operator correspondence, most of the computations are further reduced to the evaluation of energy levels in a finite-density system described by a large-charge effective field theory, usually associated with a conformal superfluid phase. The large-charge dynamics in the nonrelativistic case is however richer -- and therefore, more challenging -- than its relativistic counterpart. In this thesis, we discuss recent progress which opened the door to many new exciting large-charge applications.

==> head/dedication.tex <==
\cleardoublepage
\thispagestyle{empty}


\vspace*{3cm}

\begin{raggedleft}
    	Wings are a constraint that makes \\
	it possible to fly.\\
     --- Robert Bringhurst\\
\end{raggedleft}

\vspace{4cm}

\begin{center}
    To my parents\dots
\end{center}



